SoRTS: Learned Tree Search for Long Horizon Social Robot Navigation

The fast-growing demand for fully autonomous robots in shared spaces calls for the development of trustworthy agents that can safely and seamlessly navigate in crowded environments. Recent models for motion prediction show promise in characterizing social interactions in such environments. Still, adapting them for navigation is challenging as they often suffer from generalization failures. Prompted by this, we propose Social Robot Tree Search (SoRTS), an algorithm for safe robot navigation in social domains. SoRTS aims to augment existing socially aware motion prediction models for long-horizon navigation using Monte Carlo Tree Search. We use social navigation in general aviation as a case study to evaluate our approach and further the research in full-scale aerial autonomy. In doing so, we introduce XPlaneROS, a high-fidelity aerial simulator that enables human-robot interaction. We use XPlaneROS to conduct a first-of-its-kind user study where 26 FAA-certified pilots interact with a human pilot, our algorithm, and its ablation. Our results, supported by statistical evidence, show that SoRTS exhibits a comparable performance to competent human pilots, significantly outperforming its ablation. Finally, we complement these results with a broad set of self-play experiments to showcase our algorithm's performance in scenarios with increasing complexity.

==> sections/introduction_v2.tex <==
\section{Introduction} \label{sec:introduction}

Unmanned Aerial Vehicle (UAV) operations have seen ansignificant increase in recent years. As a result, there is a growing demand for the development of automated technologies that can be reliably integrated into the National Airspace System \cite{day2021advancing, aurambout2019last, grote2022sharing}, enabling the concurrent use of airspace between human and autonomous aircraft. The next generation of UAVs is expected to operate in low-altitude terminal airspace, where most close-proximity interactions occur \cite{patrikar2022predicting}. Therefore, it is crucial to develop technologies that ensure the safe and seamless interaction of these autonomous systems with humans. 

Toward this end, recent works have studied the domain of General Aviation (GA) in non-towered airports in the context of socially aware motion prediction \cite{patrikar2022predicting, navarro2022socialpattern}, where the goal is to characterize agent-to-agent interactions in such environments. In this domain, there is no central air traffic control authority to regulate aircraft operations, making pilots solely responsible for coordinating with each other and for following guidelines established by the FAA to ensure safe and efficient operations. Building upon \cite{patrikar2022predicting, navarro2022socialpattern}, our work aims to explore this novel domain in the context of social robot navigation. 

The goal of a social robot is to synthesize decision policies that enable it to attain its goal while interacting with humans in a socially compliant manner. Furthermore, safety-critical domains like GA demand the development of competent and trustworthy robots that can properly follow navigation norms and understand social cues to guarantee \textit{seamless} and \textit{safe} interactions. While marked progress has been made within the field of social navigation \cite{mavrogiannis2021core, rios2015proxemics, tian2022safety, kruse2013human}, achieving seamless navigation among humans while balancing social and self-interested objectives remains challenging.

For instance, classical approaches for social navigation in pedestrian settings have been proposed and remain prominent baselines \cite{helbing1995social, berg2011reciprocal, mavrogiannis2022social}. Yet, their extension to other domains is often nontrivial owing to higher environmental and social complexities that are unique to each domain \cite{wang2022social}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth,trim={0cm 0cm -0cm -0cm},clip]{figures/abstract.pdf}
    \caption{The flight simulator setup for our user study. In each experiment the \user~interacts with a \alghuman~pilot, our proposed algorithm, \algsorts, and our \algablation. The figure also shows a resulting interaction between a \user~and \algsorts.}
    \ifremvspace
    \vspace{-0.5cm}
    \fi
    \label{fig:user_study_setup}
\end{figure}

Deep Reinforcement Learning (DRL) methods have also been vastly explored within the field. Under this formulation, common strategies include approximations to the policy's reward function via hand-crafted design \cite{sadigh2018planning, liu2021decentralized}, or self-play \cite{riviere2021neural, matsuzaki2022learning}. Such techniques are generally promising in settings where data is sparse or where the robot is easily distinguishable from humans. However, tuning reward parameters for homogeneous navigation among humans is challenging \cite{mavrogiannis2017socially}. Furthermore, RL-based policies are a function of the underlying simulator, often yielding undesirable behavior in real scenarios due to a lack of compatibility between the simulated environment and the real world. 

More recently, data-driven approaches have been extensively explored predominantly within the field of socially aware motion prediction \cite{rudenko2020human}. These methods aim at characterizing human behavior and interactions observed in the data, alleviating the need for reward shaping and simulation. These models have achieved promising performance, however, using them for downstream navigation is difficult as they often suffer from prediction failures \cite{farid2023task} and myopic decision-making which hurts their generalization capabilities. This potential for unsafe behavior prompts the need for robustifying models deployed in the real world.

We, thus, introduce \textit{Social Robot Tree Search (\sorts)}, an algorithm that seeks to robustify offline-learned socially aware motion prediction models for their deployment in online settings. We build \sorts~upon the insight that, in social navigation settings, the actions of one agent influence those of another, and vice-versa \cite{sadigh2018planning, hu2022active}. This type of temporally recursive decision-making has been used for modeling human-like gameplay via search-based policies \cite{silver2018general, jacob2022modeling}. Inspired by this, we propose using recursive search-based policies to augment the aforesaid prediction methods. Specifically, we use Monte Carlo Tree Search (MCTS) \cite{kocsis2006bandit} as our search policy that provides long-horizon simulations, collision checking, and goal conditioning. We then bias its tree search using a \textit{reference} module and a \textit{social} module. The former guides the long-horizon planner via reference paths and a frequency visitation map. The latter, comprised of the offline-trained motion prediction model, provides MCTS with short-horizon agent-to-agent context cues. 

% \textit{General Aviation (GA) as a Case Study.} Unmanned aerial vehicle operations have increased significantly in recent years. As a result, there is a growing demand to integrate these automated systems into the National Airspace System so as to enable the concurrent use of airspace between human and autonomous pilots \cite{day2021advancing, aurambout2019last, grote2022sharing}. Toward this goal, GA in non-towered airports has been recently framed as a motion prediction task \cite{patrikar2022predicting, navarro2022socialpattern}. In the US alone, non-towered airports make up for 96\% of the airports. In this setting, there is no central air traffic control (ATC) authority to regulate aircraft operations. Instead, pilots are responsible for coordinating with each other and for following flying guidelines to ensure safe and efficient operations. Building upon \cite{patrikar2022predicting, navarro2022socialpattern}, we treat this novel domain as a social navigation task and use it to evaluate our approach.

% We separate these two notions into two axes: \textit{navigation efficiency} and \textit{safety}. We center the design of our algorithm, as well as our evaluations around these axes. 

To evaluate our approach, we conducted a user study with 26 experienced pilots using our custom simulator framework, \xplaneros. In our study, we investigate how pilots interact with our model in a realistic flight setting. We also study their perceptions of our model's performance along the preceding axes when compared to competent human pilots. Finally, as a complementary analysis, we provide evaluations via self-play experiments in more complex scenarios. 

\textit{Statement of Contributions}:
\begin{enumerate}
    \item We study the task of social navigation in shared airspace, introducing \sorts, an MCTS-based algorithm that aims at robustifying offline-learned socially-aware motion prediction policies for downstream long-horizon navigation. 
    \item We introduce \xplaneros, a high-fidelity simulation environment for navigation in shared aerial space.
    \item Through a user study with 26 FAA-certified pilots and self-play experiments, we show that \sorts~is perceived comparably to a competent human pilot in terms of \textit{navigation efficiency} and \textit{safety} and significantly outperforms its ablation algorithm. 
\end{enumerate}

% \textit{Organization:} \Cref{sec:related_works} provides a brief review of relevant works within the field of social navigation. \Cref{sec:problem_formulation} provides preliminary background and important notation details. We provide a detailed overview of the proposed method in \Cref{sec:approach}. In \Cref{sec:setup} we describe our high-fidelity simulator, the details of our user study and self-play experiments. We also provide details about the quantitative metrics used during the evaluation, our baseline algorithm, and specific hyperparameter and implementation details of our approach. We extensively discuss our findings in section \Cref{sec:results}. Finally, we discuss lines of future work in \Cref{sec:conclusions}. 
